Discrete Games in Endogenous Networks: Equilibria and Policy

In games of friendship links and behaviors, I propose $k$-player Nash stability---a family of equilibria, indexed by a measure of robustness given by the number of permitted link changes, which is (ordinally and cardinally) ranked in a probabilistic sense. Application of the proposed framework to adolescents' tobacco smoking and friendship decisions suggests that: (a.) friendship networks respond to increases of tobacco prices and this response amplifies the intended policy effect on smoking, (b.) racially desegregating high-schools, via stimulating the social interactions of students with different intrinsic propensity to smoke, decreases the overall smoking prevalence, (c.) adolescents are averse to sharing friends so that there is a rivalry for friendships, (d.) when data on individuals' friendship network is not available, the importance of price centered policy tools is underestimated.

==> ctrf_antismoking_raw.tex <==
\begin{table}
\centering
\begin{tabular}{cccccc}
Campaign size (\%) & Prevalence & Predicted proportional & Predicted fix net & Actual effect & Multiplier factor \\
0.0 & 46.4 & 0.0 & 0.0 & 0.0 & - \\
1.0 & 44.7 & 0.5 & 2.9 & 1.7 & 3.7 \\
2.5 & 40.7 & 1.2 & 8.2 & 5.7 & 4.9 \\
5.0 & 35.7 & 2.3 & 12.4 & 10.6 & 4.6 \\
10.0 & 29.0 & 4.6 & 18.1 & 17.4 & 3.7 \\
20.0 & 20.6 & 9.2 & 25.7 & 25.7 & 2.8 \\
30.0 & 16.4 & 13.8 & 29.7 & 29.9 & 2.2 \\
50.0 & 9.7 & 23.0 & 36.3 & 36.7 & 1.6 \\
\end{tabular}
\caption{Spillovers}
\label{table:ctrf-spillovers}
\end{table}


==> networks_01b_intro_tobacco.tex <==
%Arguably, human beings are a product and a creator of their social environments. In particular, humans engage in a complex system of social relations, also known as social interactions, which define their social environment, impact their socio-economic choices and affect the market outcomes. It is not in any way apparent, however, \emph{what} determines individuals' social environment - the social relations one is involved in - and \emph{how} this environment is interrelated with individuals' socio-economic choices. To address these questions I propose a unified framework for the analysis of individuals' behavior in the presence of endogenous social networks and I structurally estimate it with data on teen smoking decisions.

%Arguably, human beings are a product and a creator of their social environments. In particular, humans engage in a complex system of social relations, also known as social interactions, which determine their social environment, impact their socio-economic choices and affect the market outcomes. Friendships are a typical example of social relations. As such, friendships have been often pointed as a major driving force behind a wide range of individuals' decisions and social outcomes. More generally, social interactions involve ``two or more people mutually oriented towards each other's selves, that is, any behavior that tries to affect or take account of each other's subjective experiences or intentions``.\footnote{R.J. Rummel ``Understanding Conflict and War: The Conflict Helix``, John Wiley $\&$ Sons Inc (July 28, 1976).} It is then a fundamental question, into the nature of human beings, what determines individual's social environment - the social relations one is involved in - and how this environment is interrelated with individual's socio-economic choices. This duality of social environment and individual choices is the topic of this research.

%This paper develops a modeling framework for analyzing individuals' choices in the presence of endogenous social networks and implements it with data on teen smoking decisions and friendship networks.  It extends previously available frameworks, which either model choices taking the social network as given, or model network formation without incorporating additional choices.\footnote{See the surveys in \cite*{blume_brock_durlauf_ioannides_10}, \cite{jackson_08}, and \cite{jackson_zenou_12}.}  In this paper, individuals make strategic decisions both regarding their friendship relations and their actions (e.g. to smoke). In the context of a large population game, I introduce a spectrum of solution concepts, which subsume Nash equilibrium and which gradually relax the assumptions of rationality and coordination underlying Nash play. I show how the strategic interactions of the static one-shot play are embedded in an evolutionary model of network formation, which I estimate with social network data from US high schools.The proposed model can explain prominent features of social networks, such as the tendency of agents who make similar choices to be friends and the fact that individuals who share a common friend are usually friends themselves. The estimated model is used to understand the determinants of teen smoking, including the effects of friendship networks, family background, tobacco prices, and high school composition with respect to grade and race. Simulations are also performed to assess the size of the estimation bias that would arise from neglecting the endogeneity of friendship networks or not accounting for individual unobservable heterogeneity.


\input{networks_00_abstract.tex}

A substantial body of social science research examines how social interactions shape individual behavior and, more specifically, how peer networks mediate individual choices. The issues of identification and estimation of social interaction models have been analyzed in a variety of settings, including models of local interactions (i.e., only the effects of immediate friendships are accounted for) and/or global interactions (only the effects of average intra-group behavior are accounted for).\footnote{See \cite{brock_durlauf_01a,brock_durlauf_07,krauth_05b}; the more recent work of \cite*{bramoulle_djebbari_fortin_09,calvo-armengol_patacchini_zenou_09, degiorgi_pellizzari_redaelli_10}; and the survey in \cite*{blume_brock_durlauf_ioannides_10}.} As result, the main identification challenges on the empirical work with social interactions models are well understood. In particular, the correlation between an individual's choices and those of her peers may work through three channels (\citealp{manski_93}). An individual's choices may be directly influenced by the choices of her peers (endogenous effects) or by characteristics of her peers (contextual effects). In addition, the correlation between individuals' choices in a group may be due to common unobservable group-level factors (correlated effects). In this paper, I argue that to fully understand the nature of social interactions and address the issues of identifying self-selection into peer networks, we must model the co-evolution of social networks and individual behavior.

The model has the following basic features. Individuals' payoffs from smoking and friendships depend on the decisions of friends as well as on the decisions of the overall population. For a population of size $n$, I define the notion of $k$-player Nash stability as follows: In a $k$-player Nash stable network state, any subset of $k$ players is in a Nash equilibrium of the game between them when only the friendships between the $k$ players are decided together with their action statuses. Consequently, in a $k$-player Nash stable network state, no player has an incentive to alter simultaneously $k-1$ of his friendships and his action. For $k<n$, this equilibrium notion imposes less rationality than Nash equilibrium play (i.e., when $k=n$) and is, therefore, a more tenable assumption in relatively large population games. However, $k$-player Nash stability suffers well known deficiencies, on which \cite*{kandori_mailath_rob_93} remark:
\begin{quote}
While the Nash equilibrium concept has been used extensively in many diverse contexts, game theory has been unsuccessful in explaining \emph{how} players know that a Nash equilibrium will be played. Moreover, the traditional theory is silent on how players know \emph{which} Nash equilibrium is to be played if a game has multiple equally plausible Nash equilibria.
\end{quote}

To address the above concerns I develop an ``evolutionary'' model of network formation, motivated by a long line of theoretical work in evolutionary game theory.\footnote{See the seminal papers of \cite{foster_young_90}, \cite{kandori_mailath_rob_93}, and \cite{blume_93}. Some of the ideas I exploit are encountered in \citet[Chapter VII]{cournot_1838}.} In the model the network configuration arises as the outcome of agents' optimal behavior over time rather than as the instantaneous outcome of a one-shot game with many players. More specifically, in every period an individual meets $k-1$ potential friends and decides whether or not to befriend each of them and whether to revise her action status. I demonstrate that this decentralized adaptive behavior reaches a $k$-player Nash stable state in finite time. In the presence of transient preference shocks, however, the $k$-player meeting process induces a stationary distribution on the set of all possible network states. With the assumption that the preference shock follows the Gumbel distribution,\footnote{It is also known as the extreme value type I and the log-Weibull distribution.} I show that the stationary distribution induced by the network formation model is invariant to the choice of $k$. This invariance warrants the use of the stationary distribution as a behaviorally grounded statistical device to probabilistically rank the equilibria in the family of $k$-player Nash stable states.

It is important to emphasize that the goal of this paper is not to extend the evolutionary approach to the current settings, but rather to empirically study the strategic interactions that prevail in social networks through an evolutionary model of network formation. More specifically, I show how the strategic interactions of the static one-shot play are embedded in a behavioral model where the network evolves over time. Indeed, in the evolutionary model a $k$-player Nash equilibrium receives the highest probability among all the states in its immediate neighborhood. I also use the stationary distribution to structurally estimate a model of adolescent smoking and friendships.

Direct estimation of the model through maximum likelihood is computationally infeasible.\footnote{Evaluation of the likelihood for a given set of parameters requires the calculation of an intractable normalizing constant--a summation with $2^{n^2}$ terms. For networks of size $10$, this summation involves $2^{100}$ terms.} Instead, I approximate the likelihood via Markov chain Monte Carlo methods, introduced by \cite{geyer_thompson_92}. The model is estimated with data on smoking behavior, friendship networks, and home environment (parental education background and parental smoking behavior) from the National Longitudinal Study of Adolescent Health. This is a longitudinal study of a nationally representative sample of adolescents in the United States, who were in grades $7$--$12$ during the $1994$--$95$ school year.

% of social and home environment first sentence
%HOW you identify contextual vs endogenous effect - non-linearities vs exclusion restrictions. what effects are modeled and what are NOT modeled.
%Identification what is identified and why?

The estimation results indicate a substantial role for the social environment in shaping adolescents' smoking decisions. In particular, their conditional probability of smoking increases with an additional smoking friend by $7.2$ percentage points (ppt) for $7$th and $8$th graders, and $6.1$ ppt for those in grades $9$ to $12$. In addition, students in a school where $50\%$ of the whole population smokes (independently of their friendship statuses) are $15.2$ ppt more likely to smoke versus those students in a school with no smokers at all. The estimated marginal effect of various dimensions of the home environment is substantial as well. The presence of a smoker in the household increases (on average) the likelihood of an adolescent smoking by $18.5$ ppt. If the pupil's mother has completed high school or college, this likelihood falls (on average) by $5.7$ or $7.9$ ppt respectively.

I use the estimated model to perform a number of counterfactual experiments. First, I analyze how changes in the racial composition of schools affect adolescent smoking. Simulations from the model suggest that redistributing students from racially segregated schools into racially balanced schools decreases the overall smoking prevalence. Second, I use the model to document similar effects on the overall smoking when students are segregated by grades within schools (e.g., middle school and high school students are separated), which prevents friendship links between younger and older students. Third, I examine the possibility of cascade effects from anti-smoking campaigns, and find that even if substantial percentage of students are not directly exposed to the campaign, it can still have a large impact on the overall prevalence of smoking. Fourth, I examine the elasticity of adolescent smoking to varying levels of changes in tobacco prices. Finally, I compare the predictions made by the model when friendship networks are allowed to adjust to the proposed interventions against the model's predictions when friendship networks are not allowed to adjust. The simulations suggest that neglecting the endogeneity of the friendship network leads to a downward bias of $10\%$ to $15\%$ on the predicted effect of these policies on adolescent smoking rates.


%-----------------------------------------------------------------------
%-----------------------------------------------------------------------
%\subsection*{Relation to the literature}
%\subsection*{Related literature}
The literature on social interactions can be grouped into two broad classes of studies. One class of studies develops social interaction models that take the network structure as given. These range from models that directly relate an individual's choices to mean characteristics of his peer groups\footnote{See for example \cite{powell_tauras_ross_05}, \cite{ali_dwyer_09}, and the references therein. A reduced form approach to social interactions, such as the one adopted in these studies, suffers severe identification issues \citep*{manski_93}. Moreover, the empirical analysis from such studies often is not generalizable to changes in the policy environment, which are likely to operate through the social network. See the next footnote.} to models with elaborate equilibrium micro-foundations, such as those in \cite*{brock_durlauf_01a,brock_durlauf_07,krauth_05b,calvo-armengol_patacchini_zenou_09,degiorgi_pellizzari_11,bisin_moro_topa_11}. Another large literature, mostly theoretical, focuses on the strategic interactions behind network formation abstracting from any other individual choices. \cite*{jackson_wolinsky_96,bala_goyal_00,dutta_05}; and \cite{mele_10} are prominent papers in this literature.\footnote{For the moment, I abstract from a large statistical literature which approaches the network from a purely stochastic view, e.g., in their settings, the network links are formed and dissolved at random according to some probability distribution (See \citealp{reka_barabasi_02}). A similar perspective is shared by \cite{goldsmith-pinkam_imbens_11} and \cite{hsieh_lee_11}, who propose econometric models of networks and actions. Overall these models lack the equilibrium microfoundation of the strategic models of network formation, limiting their scope for policy analysis.} Depending on the specific context, conditioning the model on the peer network or focusing only on network formation may be appropriate, but to study adolescent smoking and high school friendship networks it is necessary to model these two decisions jointly.

A handful of theoretical papers consider both network formation along with other choices potentially affected by the network (See \citealp{jackson_watts_02b,goyal_vega-redondo_05,staudigl_11,staudigl_12,koenig_tessone_zenou_12}). The theoretical frameworks available, however, are meant to provide focused insights into isolated features of networks and have sharp predictions, but are not easily adapted for estimation.\footnote{\cite*{koenig_tessone_zenou_12} presents an interesting exception. They analyze a dynamic model of network formation with endogenous actions which is capable of generating the so-called nested split graph. In addition they obtain analytic characterizations of network statistics. Their model, however, is not directly applicable to the analysis of social interactions in that it does not accommodate heterogeneity of players and takes the link destruction process exogenously.} In particular, the prevailing perspective has been to use stochastic dynamics, where uncertainty vanishes as time goes by, as an equilibrium selection device, and to study conditions under which the selected (stochastically stable) states are unique, risk dominant, or efficient. As opposed to obtaining a sharper prediction, my approach is to use the uncertainty of a behavioral model of decision making to probabilistically rank the possible network states. In addition, I examine the behavioral dynamics of the network in relation to a broader class of equilibria of the static one-shot play.

Typically models of social interactions consider a situation where agents' payoffs (and hence optimal decisions) depend on the actions of other agents. Such environments have been formalized as discrete games---an extension of discrete choice models allowing for strategic interdependence of agents' payoffs.\footnote{Discrete games have been used in a variety of contexts including firms' market entry decisions \citep*{bresnahan_reiss_90,berry_92}, firms' product quality choice \citep*{mazzeo_02}, and individuals' decisions in the presence of peer effects \citep*{brock_durlauf_01a,bisin_moro_topa_11} among others.} Multiplicity is a common problem in discrete games of complete information, and extant approaches to deal with it include: modeling the outcomes that are unique even in the presence of multiplicity %\footnote{The problem of multiplicity of equilibria has been pointed much earlier than the first proposed solutions. See for example \cite{heckman_78}.}
\citep*{bresnahan_reiss_90,berry_92}, imposing an order of moves \citep*{berry_92}, assuming an ad-hoc equilibrium selection rule \citep*{hartmann_10}, obtaining the identified set estimates \citep*{tamer_03,ciliberto_tamer_09}, empirically estimating an equilibrium selection rule \citep*{bajari_hong_ryan_10}, and conditioning on the observed equilibrium (i.e. being agnostic about the equilibrium selection mechanism; \cite{bisin_moro_topa_11}).\footnote{In a recent work, \cite{narayanan_11} takes a Bayesian perspective to the problem of multiplicity. There, the prior reflects the analyst's uncertainty about equilibrium selection. His approach goes beyond estimating the identified set in that the posterior may localize high density regions within the interval estimates and thus provide more information about the parameters.} In contrast, this paper proposes a behavioral model of network formation which can address the indeterminacy of the static framework, and yet embeds the strategic incentives from the static play. In particular, the proposed model delivers a probabilistic ranking of the equilibria in the family of $k$-player Nash stable states.

Finally, this paper is related to a large body of empirical work on social interactions and risky teen behaviors. Of this literature, the closest to this work is \cite{nakajima_07}, which estimates a model of smoking decisions in an exogenously-given peer groups. In his setting, individuals sequentially update their smoking decisions, taking into account the overall smoking prevalence in the peer group they belong to. Another related work, albeit from a different point of view, is \cite{mele_10}. He developes a model of network formation in which individuals update their best friends over time, and proposes an implementation strategy via Bayesian methods. Lastly, there is a literature which uses laboratory experiments and quasi-experiments, such as exogenous assignment to peer groups, to document the presence of social effects on a wide range of behaviors.\footnote{See \cite{sacerdote_01} and the review in \cite{durlauf_ioannides_10}.} However, there are well known limitations on the interpretation of these estimates as local treatment effects (\citealp{heckman_vytlacil_05}). Moreover, these frameworks are not generalizable to peer effects outside the specific context of the experiment.\footnote{See \cite{durlauf_ioannides_10} for discussion.}


\subsection*{Background on tobacco smoking}

Tobacco is the single greatest preventable cause of death in the world today.\footnote{The World Health Organization, \emph{Report on the Global Tobacco Epidemic} ($2008$). The statistics for the U.S. are compiled from reports by the Surgeon General ($2010$), National Center for Health Statistics ($2011$), and Monitoring the Future (2011).} In the United States alone, cigarette smoking causes approximately $443,000$ deaths each year (accounting for one in every five deaths) and imposes an economic burden of more than $\$193$ billion a year in health care costs and loss of productivity. Approximately $1$ million young people under $18$ years of age start smoking each year; about $80\%$ of adults who are smokers started smoking before they were $18$ \citep*{kessler_etal_96,liang_chaloupka_nichter_clayton_01}. Despite an overall decline in smoking prevalence from $2005$ to $2010$, when the percentage of current smokers decreased from $20.9\%$ to $19.3\%$, the reduction in teen smoking has been less pronounced. In fact, the proportions of $8$th and $10$th graders who smoke increased slightly in $2010$. As with many human behaviors, social interactions (peer influence) have often been pointed to as a major driving force behind adolescent smoking choices.

Figure \ref{fig:intro} illustrates the relationship between friendships and smoking in the data sample used for the estimation. The left panel displays the smoking mixing matrix, which groups friendship nominations with respect to the smoking status of the nominator and the nominee. For example, the top left number in the table, $304$, is the number of friendships in which a smoker nominates a smoker. On the other side, $418$ is the number of friendship nominations in which a smoker nominates a non-smoker. If friendships were drawn at random then smokers and non-smokers would be nominated in proportion reflecting the size of the two groups in the sample. Clearly smokers are biased in their nominations, because $42\%$ of their friends smoke, while only $21\%$ of the sample does so. To understand the extent to which the magnitude of this correlation is unusual, the right panel of Figure \ref{fig:intro} compares friendship patterns across different socio-demographic groups. In particular, the diagram plots the Freeman segregation indexes (FSI) for sex, race, and smoking. A higher value implies a low likelihood that two individuals from different groups are friends. A value of $1$ implies no friendships between the different groups. Clearly, the segregation behavior of individuals with respect to smoking is comparable to that of race and gender.

\begin{figure}[t]
\begin{centering}
\caption{Smoking and Friendships}
\hspace{-0.0cm}
\begin{minipage}[c]{0.48\textwidth}
\centering
\begin{footnotesize}
\begin{tabular}{llcc}
  &  & \multicolumn{2}{c}{\tiny NOMINEE} \\
  \multirow{5}{*}{\rotatebox[origin=c]{90}{\tiny NOMINATOR}}
  &            & Smoker               & Nonsmoker           \\ \cmidrule{2-4} \morecmidrules \cmidrule{2-4}
  & Smoker     & \textbf{42\% (304)} &  58\% (418)          \\
  & Nonsmoker  & 16\% (499)          & \textbf{84\% (2562)} \\  \cline{2-4}
\end{tabular}%
\end{footnotesize}
\end{minipage}
\begin{minipage}[c]{0.05\textwidth}
\end{minipage}
\begin{minipage}[c]{0.5\textwidth}
  \includegraphics[width=0.98\textwidth]{../diagrams/FSI.pdf}
\end{minipage}
\end{centering}
\label{fig:intro}
\fignotetitle{Source:} \fignotetext{The National Longitudinal Study of Adolescent Health (Add Health) - Wave I, 1994-95 school year (Estimation sample: $14$ schools, $1,125$ students, $21\%$ smokers).}
\end{figure}



The rest of the paper is organized as follows. Section 2 develops the theoretical framework, which Section 3 extends to an estimable empirical model. Section 4 presents the data, the estimation method, and the parametrization of the model. In Section 5, I discuss the empirical results together with the model fit. Section 6 concludes.


